STULL: Unbiased Online Sampling for Visual Exploration of Large Spatiotemporal Data

Online sampling-supported visual analytics is increasingly important, as it allows users to explore large datasets with acceptable approximate answers at interactive rates. However, existing online spatiotemporal sampling techniques are often biased, as most researchers have primarily focused on reducing computational latency. Biased sampling approaches select data with unequal probabilities and produce results that do not match the exact data distribution, leading end users to incorrect interpretations. In this paper, we propose a novel approach to perform unbiased online sampling of large spatiotemporal data. The proposed approach ensures the same probability of selection to every point that qualifies the specifications of a user's multidimensional query. To achieve unbiased sampling for accurate representative interactive visualizations, we design a novel data index and an associated sample retrieval plan. Our proposed sampling approach is suitable for a wide variety of visual analytics tasks, e.g., tasks that run aggregate queries of spatiotemporal data. Extensive experiments confirm the superiority of our approach over a state-of-the-art spatial online sampling technique, demonstrating that within the same computational time, data samples generated in our approach are at least 50% more accurate in representing the actual spatial distribution of the data and enable approximate visualizations to present closer visual appearances to the exact ones.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> analyticsViaSTULL.tex <==
% \section{Spatiotemporal Analytics via Sampling} \label{sec:data-aggregation-analytics}

In visual analytics applications, users typically conduct operations to aggregate data across multiple dimensions.
Data aggregate functions assist end users in summarizing trends and patterns of data. 
This section introduces data aggregation computation with samples retrieved by \texttt{STULL} and estimates the accuracy of the generated approximate answers (i.e., confidence interval~\cite{lohr2009sampling}).
% for three types of spatiotemporal data analytics, including 1) general data aggregation, 2) spatial specific data aggregation, and 3) incremental data visualization. 

% \texttt{Online Temporal Aggregation}
%\label{sec:temporal-dim-estimation}


% \texttt{Online Spatial Data Aggregation}
%\label{sec:kde-estimation}

% The most common type of spatial analysis is spatial data aggregation, e.g., resource allocation of police force per spatial distribution of criminal incidents, with the focus on locations with high densities.
% This section details the use of \texttt{STULL} in constructing approximate heatmaps, a popular visual representation for spatial aggregation (Figure~\ref{fig:increvis-osp}). Note that estimation of sample sizes per the accuracy requirements on such a spatial heatmap is complicated and beyond the scope of this paper.

% Spatial heatmaps use Kernel Density Estimation (KDE)~\cite{doi:10.1137/1114019} to model the data distribution and color shades to encode KDE values on a map.
% The KDE method splits the queried spatial range into rectangular cells on a two-dimensional grid.
% Each cell is associated with a KDE value that is derived from the count of data items in the associated spatial range.
% The approximate heatmap is the color rendering result of such grid.
% Therefore, prior to constructing the approximate heatmap, we need to estimate the number of points within each cell.


% Suppose a sample set $S$ is obtained by Algorithm~\ref{algo:in-memory-sampling} for a query $Q$. $S= S_1 \cup S_2 \cup \cdots \cup S_{|T_Q|}$, where $T_Q$ is the set of temporal bins that overlap with $Q$ and $S_i$ is a set of data points sampled from the $i$-th temporal bin of $T_Q$.
% $N = \{N_1, N_2, \cdots,N_{|T_Q|}\}$ is a collection of data subsets, where $N_i$ is the data subset from which the retrieval process obtains $S_i$ in the $i$-th temporal bin. The calculation of $N_i$ is introduced in Section~\ref{sec:count-query}.
% Let $G = \{G_1, G_2,\cdots, G_{|T_Q|}\}$ be the set of grids with the same spatial divisions, where $G_i$ stores the data count in each cell based on $S_i$.
% The value in the $(i,j)$-th cell, $G(i,j)$ equals $\sum_{i=1}^{|T_Q|} G_i(i,j)\frac{|N_i|}{|S_i|}$.
% Thus, $G$ will be the final grid used by the KDE method to construct the approximate heatmap.



% Our sample retrieval procedure provides $(100\alpha\beta)$\% data points per visual update.
% Algorithm~\ref{algo:in-memory-sampling} consecutively retrieves data samples in units of while loops (in Line 14-17) and each while loop obtains $(100\alpha\beta)$\% points on average that satisfy the query.
% As a result, points obtained in one loop can be computed to generate one visual update, and it takes in total $\frac{1}{\alpha\beta}$ visual updates to fetch all data.
% For example, if $\alpha=0.25$ and $\beta = 0.2$, \texttt{STULL} will obtain 5\% records per visual update and produce a total of $\frac{1}{0.25 \times 0.2}$ visual updates from the beginning to when 100\% points are retrieved.


% The well-tuned parameter $\beta$ helps end users determine the number of points retrieved in one visual update.
% We may adjust the number of visual updates through changing either $\alpha$ or $\beta$. 
% However, changing $\alpha$ means rebuilding the data index (in Algorithm~\ref{algo:build-sample-buffer}), which is computationaly expensive.
% Instead, $\beta$ can be used as an input parameter of Algorithm~\ref{algo:in-memory-sampling}, since it would not trigger additional computations upon changes.
% Smaller $\beta$ should be used when querying relatively large data for faster responses and vice versa.


% \subsection{General Data Aggregation}
% \label{sec:count-query}

% We elaborate on the computation of sampling data from \texttt{STULL} to construct approximate answers for two common data analysis aggregate functions functions, \texttt{COUNT} and \texttt{AVG}. 


% % \subsubsection{COUNT-based Queries}
% % \label{sec:count-query}

% COUNT-based queries estimate the total number of data records satisfying particular filter conditions.
% For example, crime analysts often issue SQL queries in the format ``select COUNT(*) from table\_name where condition'' to find out incident frequencies in their cities.
% We show constructing approximate answers to such queries in two cases: 1) a query whose temporal range overlaps with one temporal bin per data index, and 2) a query whose range overlaps with multiple temporal bins.

% Constructing approximate answers to a COUNT query of one temporal bin depends on three variables, $N$, $N_a$ and $N_{a,Q}$. 
% $N$ is the size of the data subset from which Algorithm~\ref{algo:in-memory-sampling} randomly accesses $N_a$ data points. 
% And of the $N_a$ points there are $N_{a,Q}$ points satisfying specification of a given query, Q.
% According to Algorithm~\ref{algo:in-memory-sampling}, when the sample retrieval procedure stops, cells related with elements stored in the array $G$ indicate the spatiotemporal range from which the sample retrieval process obtain samples.
% Thus, $N = \sum_{c=1}^{|G|} d_c$, where $d_c$ is the data size of the cell related with the $c$-th element in $G$.
% Algorithm~\ref{algo:in-memory-sampling} starts from a random level $l_0$, goes downward and stops at a intermediate or bottom level, which is equivalent to that the sample retrieval process randomly pick $\alpha \beta N$ data from $G$ in each while loop.
% Thus, $N_a = d \times \alpha \times \beta \times N$, where $d$ is the number of while-loop runs when a sample of $N_{a,Q}$ data is retrieved.
% Equation~\ref{eq:count-estimation} shows the estimated answer $\bar{Y}$.

% \begin{equation}
% \Bar{Y} = N_{a,Q}\frac{N}{N_a} = N_{a,Q}\frac{1}{d\alpha\beta}
% \label{eq:count-estimation}
% \end{equation}

% If a query involves a set of temporal bins $T_Q$, the count estimation over $T_Q$ is $\sum_{t=1}^{|T_Q|} \Bar{Y_i}$, where $\Bar{Y_i}$ is the estimated count in the $t$-th bin of $T_Q$ according to Equation~\ref{eq:count-estimation}.

% % \subsubsection{AVG-based Queries}
% % \textcolor{orange}{merge with the previous subsection}

% % Another common query in VA is measuring the average of selected data points.
% % e.g., querying the averaged temperature of Chicago in the past 10 years.
% % \texttt{AVG} queries are typically described in the form ``select AVG(*) from table\_name where condition''.
% % Suppose a sample of $n$ points is obtained by \texttt{STULL} from a large dataset, in response to $Q$. The estimated value is then $\Bar{Y_n} =\frac{1}{n}\sum_{i=1}^{n} f(i)$, where $f(i)$ is the value of the $i$-point in the sample.
% % The confidence interval of the query follows the work~\cite{Hellerstein:1997:OA, lohr2009sampling} to be 
% % $\epsilon = z_{p/2}\sqrt{1-n/N}\sqrt{[\sum\limits_{i=1}^{n}(f(i)-\bar{Y_n})]/[n(n-1)]}$, where $N$ is the number of points in the dataset satisfying the predicate and  $z_{p/2}$ is the $(1- p/2)$-th percentile of the standard normal distribution with mean 0 and variance 1.
% % In the case where there is no knowledge of $N$, Section~\ref{sec:count-query} provides a method to estimate $N$. Further, if the sample is selected from a large dataset, $\sqrt{1-n/N}$ can be approximated as 1~\cite{Hellerstein:1997:OA}.
% % This indicates that with the probability $100(1-p)\%$, the exact answer is within the interval $[\bar{Y} - \epsilon, \bar{Y} + \epsilon]$.

% % Likewise, accuracy demands imposes sample size requirement.
% % Suppose the tolerable marginal error is $\epsilon$ and the probability is $100(1-p)\%$, Equation~\ref{eq:avg-sample-size}~\cite{lohr2009sampling} determines $n$, the minimal number of data points needed for a theoretical guarantee that $P(|\bar{Y} -\mu|\leq \epsilon) = 1-p$, where $\mu$ is the exact answer.
% % Let $[f_{min},f_{max}]$ denote the lower and upper bounds for values in a data point.
% % Since the maximal value of variance $S^2$ is $(f_{min} -f_{max})^2$, $n$ is determined to be $\frac{z_{p/2}^2}{\epsilon^2}(f_{min} -f_{max})^2$.
 
% % \begin{equation}
% % \begin{split}
% % &n = \frac{z_{p/2}^2 S^2}{\epsilon^2 + z_{p/2}^2 S^2/N} 
% % \Rightarrow n \leq \frac{z_{p/2}^2 S^2}{\epsilon^2} \\
% % &\text{ where }S^2 \text{ is the variance}
% % \end{split}
% % \label{eq:avg-sample-size}
% % \end{equation}




% \subsection{Incremental Data Visualization}
% \label{sec:incre-vis-analytics}

% \textcolor{orange}{merge with the previous subsection}

% Incremental visualization provides end users with approximate query answers at interactive rates, and progressively uses more data samples to improve the confidence and accuracy of approximate answers.
% The incremental visual update will continue until users stop it or all data have been retrieved to generate the exact visualization.
% Figure~\ref{fig:increvis-osp} shows the incremental visualization of spatial heatmaps using \texttt{STULL}.
% Computational details of the heatmap are introduced in Section~\ref{sec:kde-estimation}.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> performance.tex <==
\section*{Appendix A: Computational Performance of \texttt{STULL}}

Here we provide a formal computational performance evaluation of \texttt{STULL} through time complexity analyses for data indexing and sample retrieval.

\section*{A.1 Index construction and update}
\label{sec:data-organization-complexity}

Given a data set of $N$ points, \texttt{STULL} first takes O$(N \frac{1}{\alpha})$ to put all points into the right temporal bins and go through a $\frac{1}{\alpha}$-length path to put each point into the right leaf. Next, building sample buffers (Algorithm 1) includes a linear combination of two steps,
1) at the bottom level: random shuffling the circular array of one leaf having $m$ data points is O$(m)$,
hence random shuffling of leaves within all time bins is O$(N)$;
2) at other levels: each cell having $n$ points contains a sample buffer of $\alpha n$ points, and needs O$(\alpha n)$ for random shuffle; since
non-leaf cells in the same level have a total of $\alpha N$ points in their sample buffers, 
thereby, sample buffers in the same level take O$(\alpha N)$ for random shuffle.
Therefore, the time complexity to save data into sample buffers is O$(N + (\frac{1}{\alpha}-1)\alpha N)$ = O$((2-\alpha)N)$. To conclude, the complexity of index construction is O$(N \frac{1}{\alpha}) +$ O$((2-\alpha)N)=$ O$((2+\frac{1}{\alpha}-\alpha)N)$. 


In the case of streaming data, suppose the newly arrived data has $n$ points.
Let $M$ be the set of temporal bins that will insert new data, and a total of $N_M$ points have been indexed in the bins of $M$.
\texttt{STULL} takes O$(n\frac{1}{\alpha})$ to put all points into the right bins and leaf cells, and takes to build same buffers is O$((2-\alpha)(n+N_m)$.
As such, the time complexity to index new data is O$((2-\alpha)(n+N_m)+n\frac{1}{\alpha} )=$ O$((2+\frac{1}{\alpha}-\alpha)n+(2-\alpha)N_M)$.
From the time complexity, we can see that the performance of indexing newly arrived data relates strongly to $N_M$.
Since continuous data streams often provide data with the up-to-date time values, therefore, temporal bins that contains new points tend to be the ones belonging to the latest time range.
If the time interval of temporal bins is relatively smaller, accordingly, the total time span of bins in $M$ becomes smaller in the finer granularity of temporal bins, which further helps reduce $N_M$.
Thus, we recommend that the time interval of temporal bins in the streaming data index should be relatively smaller. 

% \textcolor{blue}{*** Guizhen to add interpretation on the performance (DSE: so what does this mean compared to other algorithms and how much real time does it take for example datasets??) ***}

% \section*{A.2 Sample retrieval}

% % Let $R_S$ be the spatial range of the entire dataset, and $R_s$ be the spatial query range specified in a query $Q$. For simplicity, we assume that $R_s \leq R_S$, because there are no points outside $R_S$.
% Suppose $\theta$ percent of points are retrieved per incremental update.
% The time complexity of retrieving $n_s$ samples from one temporal bin $m$ for $Q$ (in Algorithm 2) includes:
% (1) 
% Suppose $n_Q$ denotes the total number of points belonging to a set of leaf cells that specially range completely covering $R_s$. 
% The retrieval procedure obtains on average $\theta n_Q$ points in each round (within lines 14-17). 
% (2) It takes O($\frac{n_s}{\theta n_Q}$) rounds to retrieve $n_s$ points.

\section*{A.2 Online sample retrieval performance}

According to the sample retrieval algorithm (Algorithm 2), \texttt{STULL} retrieves on average $\theta$ percent of points satisfying $Q$ in each while loop (within lines 14-18).
Suppose $n_Q$ denotes the total number of points belonging to a set of leaf cells that spatially overlap with $Q$.
Thus, each update retrieves $n_Q\theta$ points. Thus, its time complexity is O($n_Q\theta$).
%After finishing one loop, \texttt{STULL} sends the samples and the related statistics (e.g., Confidence Interval~\cite{Hellerstein:1997:OA}) to the visualization side and continues to collect more data for the next visual update.

% Thus, in the online sampling scheme, after the visualization side specifies the expected number of data per one incremental visual update, 
% \texttt{STULL} can take one or multiple while loops in order to collect the wanted sample points.
% $\beta$ is the paramter \texttt{STULL} can adjust to determine the number of points collected in each while loop (within lines 14-17).
% For example, if each visual update wants to incorporate 1\% more data into visualizations, \texttt{STULL} uses $\beta= 1/\alpha$ to determine the percentage of retrieved data in one while loop.


==> unbiased_guarantee.tex <==
\section*{Appendix A: Unbiased Sampling Guarantee}
\label{sec:stus-unbiased-argument}
Unbiased sampling in STUS is guaranteed through the proportional sized sample buffer design and the proposed sample retrieval procedure. Here we explain and prove STUS' unbiased sampling guarantee.


\section*{A.1 Proportionally-sized sample buffer design}
The sample buffer of each cell at the non-bottom levels contains $100\alpha$ percent of the data within its specified spatio-temporal range. 
The sample buffer of each cell is therefore \textit{proportional} to the cell's specified range. 
This inherent \textbf{proportionally-sized} design provides the flexibility to approximate the distribution of the original data to guarantee unbiased sampling, whereas \textbf{fixed-sized} sampling can not.  

The issues and limits of fixed-sized buffer design are illustrated in Figure \ref{fig:storm}. In this example, each non-leaf cell has a 500-point sample buffer. At level 2, collectively, the union dataset of the orange and green cells has the distribution of $43.3\%$ (i.e. $\frac{1000+1600}{6000}$) Q1, and 56.7\% Q2, whereas the sample combining two sample buffers has the distribution of 45\% Q1, and 55\% Q2. On the contrary, proportional sized buffer design allows each cell to cache $100\alpha$ percent of its data that then aggregates to a sample containing $\alpha$ percent sample from both $Q1$ and $Q2$, leaving the distribution unaltered. 
By sampling data proportional to the categories, STUS can prevent such issue and assure the original spatial distribution is preserved.

% The issue with fixed sized buffer design is more pronounced when spatial distributions are heterogeneous for different data categories, which commonly occur in many applications. 
% For instance, when the spatial distribution of data points satisfying one category are significantly different from that of other categories, the dominant categories will dictate the spatial distribution used for the entire data set.
% When users query data categories whose spatial distribution differ from the dominant ones, the sampling bias is more significant in the fixed-size buffer design.
% Taking criminal incident data as an example, drug abuse cases~\cite{wang:vip:2017} are often one of the most frequently occurring offense types in U.S. cities, and usually concentrate in the downtown area, whereas burglary, a smaller category, tends to concentrate in residential areas during the day~\cite{wang:vip:2017}.
% A random sample of such crime incident data will largely follow the distribution of drug abuse cases rather than burglary cases.
% By sampling data proportional to the categories, STUS can prevent such issue and assure the original spatial distribution is preserved.
% In contrast, such sampling bias caused by spatial distribution heterogeneity can be avoided in our proportional-sized design.

% \textcolor{red}{Section 4.4.1 need to be further polished.}

\begin{figure}[!htb] 
  \centering
  \includegraphics[width=1\columnwidth]{storm_sampling}
  \caption{Sampling bias issue in the fixed-sized sample buffer design.
  $Q1$ and $Q2$ are two queries.
  Each sample buffer caches 500 random data points.
   Numbers inside each buffer lists the number of data points matching the particular queries. So is the numbers in each node, which denotes the total number of points in the spatiotemporal range of a cell.
  }
  \label{fig:storm}
\end{figure}


\section*{A.2 Proof of Unbiased Sampling}
\label{sec:proof}

We prove that STUS conducts unbiased sampling in two steps. First, we prove that \textsf{STUS} retrieves samples from one temporal bin without bias, and then prove for cases that use multiple bins.

For one temporal bin, $t$-th bin, the sample retrieval procedure follows Algorithm 2 to access its pyramid and obtain $n_{t,Q}$ points that satisfy $Q$.
Recall Algorithm 2, the sample retrieval procedure starts from a random level $l_0$, if $l_0 >= l_r$, and Level $\frac{1}{\alpha}$ otherwise.
The procedure in the case of $l_0 >= l_r$ is equivalent to retrieving data from the bottom level. Thus, we reduce the proof of unbiased sampling for just the bottom level.
Suppose $G_Q$ is a set of leaf cells that spatially overlap with $Q$.
In each leaf of $G_Q$, the retrieval process on average accesses $l$ segments of its circular queue, where $l=\frac{n_{t,Q}}{n_t\alpha}$ and $n_t$ is the total number of points satisfying $Q$ in the $t$-th bin.
For each leaf of $G$, the equivalent procedure first accesses the $l_0$-th circular queue segment and continues fetching data from $(l_0 +1)$-th section in a clockwise order until $l$ segments are accessed.
Equation~\ref{eq:sampling-unbias-division} shows that each segment in the circular queue of a leaf has equal chance of being selected.
Equation~\ref{eq:sampling-prob-in-one-leaf} shows $P_{\scaleto{j}{4pt}}(r_{j,Q})$, probability of picking $r$ (a data point satisfying $Q$ in the $j$-th leaf of $G_Q$), which is also the same for each point satisfying $Q$. 
Therefore, data points in each leaf of $G_Q$ are equally likely to be selected.

\begin{equation}
\begin{split}
 &P(\text{Segment $l_i$ is chosen}) = P(\text{$l_0=l_i$}) +  P(l_0 \neq l_i) \times P(l_0\\
 & \text{~~~~ belongs to } l-1
 \text{ segments counterclockwise from } l_i)\\
 &= \frac{1}{1/\alpha} + (1- \frac{1}{1/\alpha})\frac{l-1}{1/\alpha -1}
 = l\alpha = \frac{n_{t,Q}}{n_t\alpha}\alpha = \frac{n_{t,Q}}{n_t}
\end{split}
\label{eq:sampling-unbias-division}
\end{equation}

\begin{equation}
\begin{split}
&p_{\scaleto{j}{4pt}} = \sum\nolimits_{l_j=1}^{1/\alpha} P(r \text{ is in the $l_j$-th segment})\times P(l_j \text{ is chosen})\\
&= \sum\nolimits_{l_j=1}^{1/\alpha} \frac{1}{\alpha} \times \frac{n_{t,Q}}{n_t}
= \frac{n_{t,Q}}{n_t}
\end{split}
\label{eq:sampling-prob-in-one-leaf}
\end{equation}


Second, we prove that data samples retrieved from multiple temporal bins is also unbiased.
Suppose $Q$ requires data from $t_Q$ temporal bins.
$n_{Q}$ is the expected number of data samples retrieved from these $t_Q$ bins, and $n_{t,Q}$ is the expected number of data retrieved from the $t$-th bin.
$n_{t,Q}=\frac{n_{t,Q}}{\sum_{\tau=1}^{t_Q}n_{\tau,Q}} n_Q$.
From Equation~\ref{eq:sampling-prob-in-one-leaf}, we know that in the $t$-th bin the selection probability of a point satisfying $Q$ is $\frac{n_Qn_{t,Q}}{\sum_{\tau=1}^{t_Q}n_{\tau,Q}}\frac{1}{n_{t,Q}} = \frac{n_Q}{\sum_{\tau=1}^{t_Q}n_{\tau,Q}}$.
Therefore, to obtain a $n_Q$-size sample, STUS assures each point satisfying $Q$ has the same selection probability $\frac{n_Q}{\sum_{\tau=1}^{t_Q}n_{\tau,Q}}$ in any bin of $t_Q$.

In conclusion, the proposed sampling strategy is unbiased in selecting data that satisfies a multidimensional query specification.


